Multi-modal Tracking for Object based SLAM

We present an on-line 3D visual object tracking framework for monocular cameras by incorporating spatial knowledge and uncertainty from semantic mapping along with high frequency measurements from visual odometry. Using a combination of vision and odometry that are tightly integrated we can increase the overall performance of object based tracking for semantic mapping. We present a framework for integration of the two data-sources into a coherent framework through information based fusion/arbitration. We demonstrate the framework in the context of OmniMapper[1] and present results on 6 challenging sequences over multiple objects compared to data obtained from a motion capture systems. We are able to achieve a mean error of 0.23m for per frame tracking showing 9% relative error less than state of the art tracker.

==> ENP Paper/figs/algorithm/algorithm.tex <==
% \begin{algorithm}
%     \caption{Euclid’s algorithm}\label{euclid}
%     \begin{algorithmic}[1]
%         \Procedure{Euclid}{$a,b$}\Comment{The g.c.d. of a and b}
%         \State $r\gets a\bmod b$
%         \While{$r\not=0$}\Comment{We have the answer if r is 0}
%             \State $a\gets b$
%             \State $b\gets r$
%             \State $r\gets a\bmod b$
%         \EndWhile\label{euclidendwhile}
%         \State \textbf{return} $b$\Comment{The gcd is b}
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
  \caption{Object Measurement Data Association ($O$)}

  \begin{algorithmic}
   % \Statex \Comment { \%comment: acquire odometric and landmark poses\%}
    \State $I_{k}$ = Image at $k^{th}$ frame
    \State counter = 0 
    \State init = true
    \While{$I_{k}$}
        %\While{good}
        \State $T_{k}^{c,o}$  = EBT($I_{k}$,init)  
        % \EndWhile     
        \State $T_{k,k-1}$ = SVO($I_{k}$)
       % \Statex \Comment { \%comment: check measurement criteria\%}
        \If{(H($T_{k}^{c,o}$) = good)}
            \If{ Res $\leq$ $\alpha*(\sum)_{(T)^{w,o}}$ }
                \State Add $(T_{k}^{c,o})_{f}$ 
                \State counter = 0
                \State init = false
            \Else 
                \State Feedback()
            \EndIf
        \Else
            \State Feedback()
        \EndIf    
    \EndWhile
    \Function{feedback}{}
    \If{counter $\leq$ th}
        \State Reset EBT($(T_{k}^{c,o})_{e}$)
        \State counter++
        \State init = false
    \Else
        \State init = true
        \State Reset EBT(SURF)
    \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

    % \Statex \Comment { \%comment: servers[] contains the index of servers whose         data rate are sorted in descending order\%}
    % \State servers[]= index(of all servers) 
    % \State serverIndex[]=servers[0..K]
    % \State linearlyIndependentServerIndex[]=0
    % \State $[Z] \leftarrow 0$
    % \For  {$i=0$ to $serverIndex.length$} 
    % \Statex\Comment{ \%comment: find the equation corresponding the serverIndex        from the mapping at the File Server\%} 
    % \State        $eqn= equation(serverIndex[i])$ 
    % \Statex\Comment{ \%comment: try insert equation into Z using OFG\%} 

    % \EndFor end for 
    % \While{ ( linearlyIndependentServerIndex.length!=K ) } 
    % \Statex\Comment{\%comment: remove all the server index which were not inserted in Z\%}  
    % \State temp[]=serverIndex[]-linearlyIndependentServerIndex 
    % \If{  (linearlyIndependentServerIndex.length=K) }
    % \State break
    % \EndIf  
    % \EndWhile  

% \begin{algorithm}[H]
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }
%  initialization\;
%  \While{not at end of this document}{
%   read current\;
%   \eIf{understand}{
%   go to next section\;
%   current section becomes this one\;
%   }{
%   go back to the beginning of current section\;
%   }
%  }
%  \caption{How to write algorithms}
% \end{algorithm}

==> ENP Paper/figs/diagrams/factorgraphs.tex <==
\begin{figure}
        \centering
        % \begin{subfigure}[b]{0.45\textwidth}
        %     \centering
        %     \includegraphics[page=2,
        %         scale=0.20,
        %         % width=\linewidth,
        %         trim=0 30 0 30,
        %         clip]
        %         {figs/diagrams/GraphFigures}
        %     \caption{The pose of the camera at $i^{th}$ time step is $x_{i}$ with $i\in0\dots M$,
        %     a landmark is $l_{j}$ with $j\in1\dots N$ and a measurement is $z_{k}$,
        %     with $k\in1\dots K$. }
        %     \label{beliefNet}
        % \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        % \begin{subfigure}[b]{0.45\textwidth}
        %     \centering
            \includegraphics[page=3,
                scale=0.25,
                % width=\linewidth,
                trim=100 75 100 75,
                clip]
                {figs/diagrams/GraphFigures}
            \caption{The pose of the camera at $i^{th}$ time step is $x_{i}$ with $i\in0\dots M$,
            a landmark is $l_{j}$ with $j\in1\dots N$ and a measurement is $z_{k}$,
            with $k\in1\dots K$. Factor graph representation. Blue circles denote camera poses ($X$) and green circles denote landmarks ($L$). Small purple circles represent odometry constraints and red circles represent landmark-pose constraint($Z$).}
            % \label{factorGraph}
        % \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        % \caption{}
        \label{fig:factorgraph}
\end{figure}

==> ENP Paper/figs/diagrams/trackingdiagram.tex <==
\begin{figure*}
    \setlength{\abovecaptionskip}{10pt plus 3pt minus 2pt} % Chosen fairly arbitrarily
    \centering
    \includegraphics[page=2,
        width=\textwidth,
        % height=5cm,
        trim=0 0 0 205,
        clip]
        {figs/diagrams/TrackingDiagram}
    \caption{Flow diagram for proposed tracking framework. Each plugin process measurements from the same image, but commit different levels of information into the graph. With this form of cascading feedback, both plugins influence each other as they supervise their own measurement source's performance}
    \label{flowdiagram}
\end{figure*}

==> ENP Paper/figs/images/objects.tex <==
\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm]
                    {figs/images/ron/ron_color}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_grey}
        \end{subfigure}%
        \quad
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_svo}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_3d}
        \end{subfigure}
    \caption{3D model based visual tracking aided by SLAM. \textbf{(Clockwise from top left)} Original image input, the model rendered on image using pose from model based tracker, the optimized estimates for the pose and landmarks in the world frame and sparse features used for visual odometry. (Point cloud serves for visualization only.)}
    \label{fig:factorgraph}
\end{figure}


% \begin{figure}
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/Camera}
%         \end{subfigure}%
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/Edges}
%         \end{subfigure}%
%         \quad
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/SVO}
%         \end{subfigure}%
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/3D}
%         \end{subfigure}
%     \caption{Multiple 3D model-based visual trackers publish measurements used as semantic landmarks. Above \textbf{(TBLR)} is the original image input, the edge results from model based tracker, sparse features from visual odometry, and the optimized estimates for the optical pose and landmarks in the world frame; an example of multi-modal tracking for objects in low texture scenes. Point cloud serves for visualization only.}
%     \label{fig:factorgraph}
% \end{figure}


    % \setlength{\abovecaptionskip}{10pt plus 3pt minus 2pt} % Chosen fairly arbitrarily
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[page=3,
    %         % scale=0.25,
    %         width=\linewidth,
    %         trim=100 75 100 75,
    %         clip]
    %         {figs/diagrams/GraphFigures}
    %     \caption{Factor graph representation. Blue denote camera poses ($X$) and green denote landmarks ($L$). Purple represent odometry constraints and red represent landmark-pose constraint.}
    %     \label{factorGraph}
    % \end{subfigure}%
    % ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
      %(or a blank line to force the subfigure onto a new line)

% \begin{figure}
%         \centering
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Edges}
%         \end{subfigure}
%         ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Results}
%         \end{subfigure}
%         %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Camera}
%         \end{subfigure}
%         ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/3D}
%         \end{subfigure}
%         \label{fig:factorgraphs}
% \end{figure}

==> ENP Paper/figs/images/occ/occ_image.tex <==
\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_grey_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_grey_2}
        \end{subfigure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_edge_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_edge_2}
        \end{subfigure}
    \caption{Top: Object superimposed on the image , Bottom: Edge image superimposed with object. Shown above on the left is the view of the object in the Ronzoni Occlud sequence just before exiting the scene. On the right is the relocalization of the object as it comes back into view.}
    \label{fig:ron_occ}
\end{figure}

\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_grey_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_grey_1}
        \end{subfigure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_edge_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_edge_1}
        \end{subfigure}
    \caption{Top: Object superimposed on the image , Bottom: Edge image superimposed with object. Similar to Fig \ref{fig:ron_occ}, left side shows the Orange Occlud sequence just before the object exits the scene, while the right hand side shows the object being still tracked with high occlusion.}
    \label{fig:oj_occ}
\end{figure}

==> ENP Paper/figs/images/tide/tide_images.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_grey_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_edge_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_3d_1}
        \end{subfigure}
        % \quad
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_grey_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_edge_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_3d_2}
        \end{subfigure}
    \caption{Above shown are frames from the Tide sequence (Left to Right): Tracked hypotheses superimposed on the image,  the edge based error using the select edges from the object model, and finally the optimized trajectory derived from the combined SVO and object measurements. Point cloud shown is only used as visual aid. Second row shows instances of foreground occlusion.}
    \label{fig:factorgraph}
\end{figure*}

==> ENP Paper/figs/results/figures/line_plots.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ojflo_data-ojflo_data_particle-ojflo_data_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ron_data-ron_data_particle-ron_data_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/tide-tide_particle-tide_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ojflo_occ-ojflo_occ_particle-ojflo_occ_svo}
                % \caption{SVO}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ron_occ-ron_occ_particle-ron_occ_svo}
                % \caption{SVO}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/tide_occ-tide_occ_particle-tide_occ_svo}
                % \caption{SVO}
        \end{subfigure}
    \caption{Per Frame Error of objects ( Left to Right: Orange Juice, Ronzoni Box and Tide Bottle) in 6 sequences. Figures show translational error in meters over time in seconds. First row shows tracking results as the camera is moved around a cluttered table, while the second row shows out of scene occlusion comparison caused by camera rotations and translations in front of tracked object. Note the initial spike in error for EBT particle tracking just before losing the object.}
    \label{fig:error_plots}
\end{figure*}

==> ENP Paper/figs/results/result_plots.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ebt_ate}
                % \caption{Object Tracker}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/svo_ate}
                % \caption{SVO}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/omni_ate}
                % \caption{Our Approach}
        \end{subfigure}
    \caption{Shown above are views of the edge-based in low texture scene. Absolute Trajectory Errors for ronzoni box sequence (a low texture scene), shown from left to right: raw estimate for tracking and SVO measurements and our combined approach}
    \label{fig:trajectory_plots}
\end{figure*}

==> ENP Paper/figs/results/ron_19/ron_19.tex <==
\begin{figure}
        \begin{subfigure}[b]{\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ron_19/rpe_trans_error}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ron_19/rpe_rot_error}
                % \caption{SVO}
        \end{subfigure}%
    \caption{Translational and Rotational Relative Pose Error for risoni box sequence}
    \label{fig:error_plots}
\end{figure}



==> ENP Paper/figs/results/ron_19/table.tex <==
\begin{table}[]
\centering
\caption{Mean Absolute Trajectory and Relative Pose Error}
\label{my-label}
\begin{tabu}{l|[2pt]l|l|l}
risoni box sequence  & Tracker  & SVO & Approach \\ \tabucline[2pt]{-}
Mean RPE Tran [m] & 0.0907 & 0.2087 & 0.1061  \\ \hline
Mean RPE Rot [rad] & 0.14245 & 0.1778 & 0.0700 \\ \hline
Mean ATE Tran [m] & 0.0951 & 0.1001 & 0.1322
\end{tabu}
\end{table}


==> ENP Paper/figs/results/table1.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{ll|c|c|c|}
\cline{3-5}
                                                                                                 &        & \multicolumn{3}{c|}{\textbf{Method}}                                                                                                                                   \\ \hline
\multicolumn{2}{|c|}{\textbf{Sequence}}                                                                    & \textit{SVO}                                          & \textit{EBT}                                          & \textit{Approach}                                 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange\\ Juice\end{tabular}}}    & mean [m] & {\textbf{0.189}}  & 0.219  & 0.192  \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 30.10 & 21.95 & {\textbf{33.74}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange \\ Occlud\end{tabular}}}  & mean [m] & {\textbf{0.233}}   & 0.257   & 0.250   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 64.43  & 75.56  & {\textbf{82.99}}  \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Box\end{tabular}}}    & mean [m] & 0.303    & {\textbf{0.239}}    & 0.274    \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 41.37   & 23.23   & {\textbf{43.64}}   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Occlud\end{tabular}}} & mean [m] & {\textbf{0.188}}     & 0.215     & 0.197     \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 99.09    & 94.08    & {\textbf{99.59}}    \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Bottle\end{tabular}}}    & mean [m] & 0.289        & 0.288        & {\textbf{0.282}}        \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & {\textbf{41.97}}       & 30.09       & 41.25       \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Occlud\end{tabular}}}    & mean [m] & 0.210    & 0.293    & {\textbf{0.194}}    \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & {\textbf{86.89}}   & 53.15   & 85.22   \\ \hline
\end{tabular}
\caption{Per Frame Translation Error less than 0.5 m. Ratio derived from frames with error under the threshold, while mean is then derived from corresponding frames.}
\label{my-label}
\end{table}

==> ENP Paper/figs/results/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{ll|c|c|}
\cline{3-4}
                                                                                                 &            & \multicolumn{2}{c|}{\textbf{Method}} \\ \hline
\multicolumn{2}{|c|}{\textbf{Sequence}}                                                                        & \textit{SVO}     & \textit{Approach} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange\\ Juice\end{tabular}}}    & mean [m]   & 0.090 $\pm$ 0.103  & 0.119 $\pm$ 0.094   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.063            & 0.094             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange \\ Occlud\end{tabular}}}  & mean [m]   & 0.095 $\pm$ 0.062  & 0.100 $\pm$ 0.060   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.073            & 0.083             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Box\end{tabular}}}    & mean [m]   & 0.052 $\pm$ 0.028  & 0.117 $\pm$ 0.055   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.050            & 0.109             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Occlud\end{tabular}}} & mean [m]   & 0.015 $\pm$ 0.008  & 0.038 $\pm$ 0.021   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.013            & 0.030             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Bottle\end{tabular}}}    & mean [m]   & 0.135 $\pm$ 0.045  & 0.115 $\pm$ 0.053   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.126            & 0.100             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Occlud\end{tabular}}}    & mean [m]   & 0.108 $\pm$ 0.103  & 0.124 $\pm$ 0.099   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.069            & 0.083             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}All \end{tabular}}}            & mean [m]   & 0.083 $\pm$ 0.058  & 0.102 $\pm$ 0.064   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.066            & 0.083             \\ \hline
\end{tabular}
\caption{Absolute Trajectory error with respect to motion capture ground truth system. Shown is a comparison between our approach and SVO.}
\label{table:ground_truth_error}
\end{table}

==> figs/algorithm/algorithm.tex <==
% \begin{algorithm}
%     \caption{Euclid’s algorithm}\label{euclid}
%     \begin{algorithmic}[1]
%         \Procedure{Euclid}{$a,b$}\Comment{The g.c.d. of a and b}
%         \State $r\gets a\bmod b$
%         \While{$r\not=0$}\Comment{We have the answer if r is 0}
%             \State $a\gets b$
%             \State $b\gets r$
%             \State $r\gets a\bmod b$
%         \EndWhile\label{euclidendwhile}
%         \State \textbf{return} $b$\Comment{The gcd is b}
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
  \caption{Object Measurement Data Association ($O$)}

  \begin{algorithmic}
   % \Statex \Comment { \%comment: acquire odometric and landmark poses\%}
    \State $I_{k}$ = Image at $k^{th}$ frame
    \State counter = 0 
    \State init = true
    \While{$I_{k}$}
        %\While{good}
        \State $T_{k}^{c,o}$  = EBT($I_{k}$,init)  
        % \EndWhile     
        \State $T_{k,k-1}$ = SVO($I_{k}$)
       % \Statex \Comment { \%comment: check measurement criteria\%}
        \If{(H($T_{k}^{c,o}$) = good)}
            \If{ Res $\leq$ $\alpha*(\sum)_{(T)^{w,o}}$ }
                \State Add $(T_{k}^{c,o})_{f}$ 
                \State counter = 0
                \State init = false
            \Else 
                \State Feedback()
            \EndIf
        \Else
            \State Feedback()
        \EndIf    
    \EndWhile
    \Function{feedback}{}
    \If{counter $\leq$ th}
        \State Reset EBT($(T_{k}^{c,o})_{e}$)
        \State counter++
        \State init = false
    \Else
        \State init = true
        \State Reset EBT(SURF)
    \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

    % \Statex \Comment { \%comment: servers[] contains the index of servers whose         data rate are sorted in descending order\%}
    % \State servers[]= index(of all servers) 
    % \State serverIndex[]=servers[0..K]
    % \State linearlyIndependentServerIndex[]=0
    % \State $[Z] \leftarrow 0$
    % \For  {$i=0$ to $serverIndex.length$} 
    % \Statex\Comment{ \%comment: find the equation corresponding the serverIndex        from the mapping at the File Server\%} 
    % \State        $eqn= equation(serverIndex[i])$ 
    % \Statex\Comment{ \%comment: try insert equation into Z using OFG\%} 

    % \EndFor end for 
    % \While{ ( linearlyIndependentServerIndex.length!=K ) } 
    % \Statex\Comment{\%comment: remove all the server index which were not inserted in Z\%}  
    % \State temp[]=serverIndex[]-linearlyIndependentServerIndex 
    % \If{  (linearlyIndependentServerIndex.length=K) }
    % \State break
    % \EndIf  
    % \EndWhile  

% \begin{algorithm}[H]
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }
%  initialization\;
%  \While{not at end of this document}{
%   read current\;
%   \eIf{understand}{
%   go to next section\;
%   current section becomes this one\;
%   }{
%   go back to the beginning of current section\;
%   }
%  }
%  \caption{How to write algorithms}
% \end{algorithm}

==> figs/diagrams/factorgraphs.tex <==
\begin{figure}
        \centering
        % \begin{subfigure}[b]{0.45\textwidth}
        %     \centering
        %     \includegraphics[page=2,
        %         scale=0.20,
        %         % width=\linewidth,
        %         trim=0 30 0 30,
        %         clip]
        %         {figs/diagrams/GraphFigures}
        %     \caption{The pose of the camera at $i^{th}$ time step is $x_{i}$ with $i\in0\dots M$,
        %     a landmark is $l_{j}$ with $j\in1\dots N$ and a measurement is $z_{k}$,
        %     with $k\in1\dots K$. }
        %     \label{beliefNet}
        % \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        % \begin{subfigure}[b]{0.45\textwidth}
        %     \centering
            \includegraphics[page=3,
                scale=0.25,
                % width=\linewidth,
                trim=100 75 100 75,
                clip]
                {figs/diagrams/GraphFigures}
            \caption{The pose of the camera at $i^{th}$ time step is $x_{i}$ with $i\in0\dots M$,
            a landmark is $l_{j}$ with $j\in1\dots N$ and a measurement is $z_{k}$,
            with $k\in1\dots K$. Factor graph representation. Blue circles denote camera poses ($X$) and green circles denote landmarks ($L$). Small purple circles represent odometry constraints and red circles represent landmark-pose constraint($Z$).}
            % \label{factorGraph}
        % \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        % \caption{}
        \label{fig:factorgraph}
\end{figure}

==> figs/diagrams/trackingdiagram.tex <==
\begin{figure*}
    \setlength{\abovecaptionskip}{10pt plus 3pt minus 2pt} % Chosen fairly arbitrarily
    \centering
    \includegraphics[page=2,
        width=\textwidth,
        % height=5cm,
        trim=0 0 0 205,
        clip]
        {figs/diagrams/TrackingDiagram}
    \caption{Flow diagram for proposed tracking framework. Each plugin process measurements from the same image, but commit different levels of information into the graph. With this form of cascading feedback, both plugins influence each other as they supervise their own measurement source's performance}
    \label{flowdiagram}
\end{figure*}

==> figs/images/objects.tex <==
\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm]
                    {figs/images/ron/ron_color}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_grey}
        \end{subfigure}%
        \quad
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_svo}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth,height = 5cm ]
                    {figs/images/ron/ron_3d}
        \end{subfigure}
    \caption{3D model based visual tracking aided by SLAM. \textbf{(Clockwise from top left)} Original image input, the model rendered on image using pose from model based tracker, the optimized estimates for the pose and landmarks in the world frame and sparse features used for visual odometry. (Point cloud serves for visualization only.)}
    \label{fig:factorgraph}
\end{figure}


% \begin{figure}
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/Camera}
%         \end{subfigure}%
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/Edges}
%         \end{subfigure}%
%         \quad
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/SVO}
%         \end{subfigure}%
%         \begin{subfigure}[b]{0.5\linewidth}
%                 \includegraphics
%                     [width=\linewidth]
%                     {figs/images/3D}
%         \end{subfigure}
%     \caption{Multiple 3D model-based visual trackers publish measurements used as semantic landmarks. Above \textbf{(TBLR)} is the original image input, the edge results from model based tracker, sparse features from visual odometry, and the optimized estimates for the optical pose and landmarks in the world frame; an example of multi-modal tracking for objects in low texture scenes. Point cloud serves for visualization only.}
%     \label{fig:factorgraph}
% \end{figure}


    % \setlength{\abovecaptionskip}{10pt plus 3pt minus 2pt} % Chosen fairly arbitrarily
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[page=3,
    %         % scale=0.25,
    %         width=\linewidth,
    %         trim=100 75 100 75,
    %         clip]
    %         {figs/diagrams/GraphFigures}
    %     \caption{Factor graph representation. Blue denote camera poses ($X$) and green denote landmarks ($L$). Purple represent odometry constraints and red represent landmark-pose constraint.}
    %     \label{factorGraph}
    % \end{subfigure}%
    % ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
      %(or a blank line to force the subfigure onto a new line)

% \begin{figure}
%         \centering
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Edges}
%         \end{subfigure}
%         ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Results}
%         \end{subfigure}
%         %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/Camera}
%         \end{subfigure}
%         ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%           %(or a blank line to force the subfigure onto a new line)
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[
%                 width=\linewidth]
%                 {figs/images/3D}
%         \end{subfigure}
%         \label{fig:factorgraphs}
% \end{figure}

==> figs/images/occ/occ_image.tex <==
\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_grey_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_grey_2}
        \end{subfigure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_edge_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/ron_edge_2}
        \end{subfigure}
    \caption{Top: Object superimposed on the image , Bottom: Edge image superimposed with object. Shown above on the left is the view of the object in the Ronzoni Occlud sequence just before exiting the scene. On the right is the relocalization of the object as it comes back into view.}
    \label{fig:ron_occ}
\end{figure}

\begin{figure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_grey_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_grey_1}
        \end{subfigure}
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_edge_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/occ/oj_edge_1}
        \end{subfigure}
    \caption{Top: Object superimposed on the image , Bottom: Edge image superimposed with object. Similar to Fig \ref{fig:ron_occ}, left side shows the Orange Occlud sequence just before the object exits the scene, while the right hand side shows the object being still tracked with high occlusion.}
    \label{fig:oj_occ}
\end{figure}

==> figs/images/tide/tide_images.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_grey_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_edge_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_3d_1}
        \end{subfigure}
        % \quad
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_grey_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_edge_2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/images/tide/tide_3d_2}
        \end{subfigure}
    \caption{Above shown are frames from the Tide sequence (Left to Right): Tracked hypotheses superimposed on the image,  the edge based error using the select edges from the object model, and finally the optimized trajectory derived from the combined SVO and object measurements. Point cloud shown is only used as visual aid. Second row shows instances of foreground occlusion.}
    \label{fig:factorgraph}
\end{figure*}

==> figs/results/figures/line_plots.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ojflo_data-ojflo_data_particle-ojflo_data_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ron_data-ron_data_particle-ron_data_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/tide-tide_particle-tide_svo}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ojflo_occ-ojflo_occ_particle-ojflo_occ_svo}
                % \caption{SVO}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/ron_occ-ron_occ_particle-ron_occ_svo}
                % \caption{SVO}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/figures/tide_occ-tide_occ_particle-tide_occ_svo}
                % \caption{SVO}
        \end{subfigure}
    \caption{Per Frame Error of objects ( Left to Right: Orange Juice, Ronzoni Box and Tide Bottle) in 6 sequences. Figures show translational error in meters over time in seconds. First row shows tracking results as the camera is moved around a cluttered table, while the second row shows out of scene occlusion comparison caused by camera rotations and translations in front of tracked object. Note the initial spike in error for EBT particle tracking just before losing the object.}
    \label{fig:error_plots}
\end{figure*}

==> figs/results/result_plots.tex <==
\begin{figure*}
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ebt_ate}
                % \caption{Object Tracker}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/svo_ate}
                % \caption{SVO}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/omni_ate}
                % \caption{Our Approach}
        \end{subfigure}
    \caption{Shown above are views of the edge-based in low texture scene. Absolute Trajectory Errors for ronzoni box sequence (a low texture scene), shown from left to right: raw estimate for tracking and SVO measurements and our combined approach}
    \label{fig:trajectory_plots}
\end{figure*}

==> figs/results/ron_19/ron_19.tex <==
\begin{figure}
        \begin{subfigure}[b]{\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ron_19/rpe_trans_error}
                % \caption{Object Tracker}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
                \includegraphics
                    [width=\linewidth]
                    {figs/results/ron_19/rpe_rot_error}
                % \caption{SVO}
        \end{subfigure}%
    \caption{Translational and Rotational Relative Pose Error for risoni box sequence}
    \label{fig:error_plots}
\end{figure}



==> figs/results/ron_19/table.tex <==
\begin{table}[]
\centering
\caption{Mean Absolute Trajectory and Relative Pose Error}
\label{my-label}
\begin{tabu}{l|[2pt]l|l|l}
risoni box sequence  & Tracker  & SVO & Approach \\ \tabucline[2pt]{-}
Mean RPE Tran [m] & 0.0907 & 0.2087 & 0.1061  \\ \hline
Mean RPE Rot [rad] & 0.14245 & 0.1778 & 0.0700 \\ \hline
Mean ATE Tran [m] & 0.0951 & 0.1001 & 0.1322
\end{tabu}
\end{table}


==> figs/results/table1.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{ll|c|c|c|}
\cline{3-5}
                                                                                                 &        & \multicolumn{3}{c|}{\textbf{Method}}                                                                                                                                   \\ \hline
\multicolumn{2}{|c|}{\textbf{Sequence}}                                                                    & \textit{SVO}                                          & \textit{EBT}                                          & \textit{Approach}                                 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange\\ Juice\end{tabular}}}    & mean [m] & {\textbf{0.189}}  & 0.219  & 0.192  \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 30.10 & 21.95 & {\textbf{33.74}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange \\ Occlud\end{tabular}}}  & mean [m] & {\textbf{0.233}}   & 0.257   & 0.250   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 64.43  & 75.56  & {\textbf{82.99}}  \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Box\end{tabular}}}    & mean [m] & 0.303    & {\textbf{0.239}}    & 0.274    \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 41.37   & 23.23   & {\textbf{43.64}}   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Occlud\end{tabular}}} & mean [m] & {\textbf{0.188}}     & 0.215     & 0.197     \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & 99.09    & 94.08    & {\textbf{99.59}}    \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Bottle\end{tabular}}}    & mean [m] & 0.289        & 0.288        & {\textbf{0.282}}        \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & {\textbf{41.97}}       & 30.09       & 41.25       \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Occlud\end{tabular}}}    & mean [m] & 0.210    & 0.293    & {\textbf{0.194}}    \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & ratio \% & {\textbf{86.89}}   & 53.15   & 85.22   \\ \hline
\end{tabular}
\caption{Per Frame Translation Error less than 0.5 m. Ratio derived from frames with error under the threshold, while mean is then derived from corresponding frames.}
\label{my-label}
\end{table}

==> figs/results/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{ll|c|c|}
\cline{3-4}
                                                                                                 &            & \multicolumn{2}{c|}{\textbf{Method}} \\ \hline
\multicolumn{2}{|c|}{\textbf{Sequence}}                                                                        & \textit{SVO}     & \textit{Approach} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange\\ Juice\end{tabular}}}    & mean [m]   & 0.090 $\pm$ 0.103  & 0.119 $\pm$ 0.094   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.063            & 0.094             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Orange \\ Occlud\end{tabular}}}  & mean [m]   & 0.095 $\pm$ 0.062  & 0.100 $\pm$ 0.060   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.073            & 0.083             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Box\end{tabular}}}    & mean [m]   & 0.052 $\pm$ 0.028  & 0.117 $\pm$ 0.055   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.050            & 0.109             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ronzoni \\ Occlud\end{tabular}}} & mean [m]   & 0.015 $\pm$ 0.008  & 0.038 $\pm$ 0.021   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.013            & 0.030             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Bottle\end{tabular}}}    & mean [m]   & 0.135 $\pm$ 0.045  & 0.115 $\pm$ 0.053   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.126            & 0.100             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tide \\ Occlud\end{tabular}}}    & mean [m]   & 0.108 $\pm$ 0.103  & 0.124 $\pm$ 0.099   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.069            & 0.083             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}All \end{tabular}}}            & mean [m]   & 0.083 $\pm$ 0.058  & 0.102 $\pm$ 0.064   \\ \cline{2-2}
\multicolumn{1}{|l|}{}                                                                           & median [m] & 0.066            & 0.083             \\ \hline
\end{tabular}
\caption{Absolute Trajectory error with respect to motion capture ground truth system. Shown is a comparison between our approach and SVO.}
\label{table:ground_truth_error}
\end{table}
